A linear adjustment based approach to posterior drift in transfer learning

We present a new model and methods for the posterior drift problem where the regression function in the target domain is modeled as a linear adjustment (on an appropriate scale) of that in the source domain, an idea that inherits the simplicity and the usefulness of generalized linear models and accelerated failure time models from the classical statistics literature, and study the theoretical properties of our proposed estimator in the binary classification problem. Our approach is shown to be flexible and applicable in a variety of statistical settings, and can be adopted to transfer learning problems in various domains including epidemiology, genetics and biomedicine. As a concrete application, we illustrate the power of our approach through mortality prediction for British Asians by borrowing strength from similar data from the larger pool of British Caucasians, using the UK Biobank data.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\subjectto{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> extra.tex <==
\newpage
\paragraph{Outline for parametric rate}:
From the above minimization problem we have 
\[ \widehat \bE_Q \Bigg[ \nabla_w \ell \Big(  \hat w^Tx, \hat\eta_P(x)\Big)  \Bigg] = 0. \] Using Taylor's expansion up to first order term 


\[ \begin{aligned}
&\underbrace{ \widehat \bE_Q \Bigg[ \nabla_w \ell \Big(  w_*^Tx, \eta_P^*(x)\Big)  \Bigg]}_{\text{I}} + \underbrace{\widehat \bE_Q \bigg[ \nabla^2_w \ell \Big(  \tilde a(x), \eta_P^*(x)\Big)  \bigg] \big(\hat w - w\big)}_{\text{II}}  \\
& \quad + \underbrace{\widehat \bE_Q \bigg[ \nabla_{b}\nabla_w \ell \Big(  w_*^Tx,\tilde b(x)\Big) \big(\hat \eta_P(x) - \eta_P^*(x)\big)  \bigg]}_{\text{III}} = 0
 \end{aligned} \] 
 
 Here, \[  
 \begin{aligned}
 \nabla_w \ell \Big(  w^Tx, \eta_P(x)\Big) &= \bigg[\rho'\Big(a + \sigma^{-1}\big(b\big)  \Big) - y\bigg]x\\
 & = \bigg[\sigma\Big(a + \sigma^{-1}\big(b\big)  \Big) - y\bigg]x,
 \end{aligned}\]
 
 \[  
 \begin{aligned}
 \nabla^2_w \ell \Big(  w^Tx, \eta_P(x)\Big) &= \sigma'\Big(a + \sigma^{-1}\big(b\big)  \Big)xx^T\\
 & = \big\{\sigma (1-\sigma)\big\} \Big(a + \sigma^{-1}\big(b\big)  \Big)xx^T
 \end{aligned}\]
  and 
  
  \[  
 \begin{aligned}
 \nabla_b\nabla_w \ell \Big(  w^Tx, \eta_P(x)\Big) &= \sigma'\Big(a + \sigma^{-1}\big(b\big)  \Big) \big(\sigma^{-1}\big)' \big(b(x)\big) x\\
 & = \frac{e^{a+\sigma^{-1}(b)}}{\Big(1+e^{a+\sigma^{-1}(b)}\Big)^2} \frac{1}{b(1-b)}x
 \end{aligned}\] 
 Here  \[ 
 \begin{aligned}
 f(b) & =  \frac{e^{a+\sigma^{-1}(b)}}{\Big(1+e^{a+\sigma^{-1}(b)}\Big)^2} \frac{1}{b(1-b)}\\
 & = \frac{e^a \frac b{1-b}}{\Big(1+e^a \frac b{1-b}\Big)^2} \frac{1}{b(1-b)}\\
 & = \frac{e^a }{\Big((1 - b) +be^a \Big)^2}
 \end{aligned}
 \]
 
 has the derivative \[
  f'(b) = - \frac{2e^a(e^a - 1) }{\Big((1 - b) +be^a \Big)^3} = \begin{cases} \le  0 & \text{ if }a\ge 0\\
 \ge 0 & \text{ if } a\le 0.
 \end{cases}
 \]
 Hence, \[
  f(b) \le \left. \begin{cases} f(0) = e^a & \text{ if }a\ge 0\\
 f(1) = e^{-a} & \text{ if } a\le 0
 \end{cases}\right\}= e^{|a|}
 \]
 
 
 
%where $\tilde a(x)$ is some value between $\widehat \logit_P(x) + \hat w^T x + \hat b$ and $\logit_P(x) +  w^T x +  b.$ This can be rewritten as 
% \[\begin{aligned}
% &  \underbrace{\widehat \bE_Q \left[\left(\begin{array}{c}
%      1 \\ x
% \end{array}\right)  \left(
%      1,   x^T
% \right) \ddot \ell   \Big(  \tilde a(x), y  \Big)  \right] }_{\text{(I)}} \left(\begin{array}{c}
%      \hat b - b \\\hat w - w
% \end{array}\right) \\
% & \quad = - \underbrace{\widehat \bE_Q \Bigg[ \left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \dot \ell \Big(  \logit_P(x) +  w^T x +  b, y  \Big)\Bigg]}_{\text{(II)}} \\
% & \quad \quad- \underbrace{\widehat \bE_Q \Bigg[\left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \Big\{\widehat \logit_P(x) -  \logit_P(x)  \Big\} \ddot \ell   \Big(  \tilde a(x), y  \Big)\Bigg]}_{\text{(III)}}
% \end{aligned} \]
% To establish parametric rate for $(\hat b, \hat w)$ \begin{enumerate}
%     \item Minimum eigenvalue of (I) is bounded away from $0.$
%     \item Concentration of (II) is controlled using \[ \bE_Q \Bigg[ \left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \dot \ell \Big(  \logit_P(x) +  w^T x +  b, y  \Big)\Bigg] = 0 \] and the mean concentration. Will provide $n_Q^{-1/2}$ rate. 
% \item Concentration of (III) is controlled using concentration of $\hat P(1|x)$ which should provide $n_P^{-\frac \beta {2\beta + d}}$-rate for non-parametric estimation of $P(1|x)$, and $n_P^{-1/2}$-rate for parametric estimation. 
% \item From the above three steps the parametric rate of convergence should be \[ \begin{cases}
% n_P^{-\beta/{2\beta+d}} + n_Q^{-1/2} & \text{for non-parametric }P(1|x) \\
% n_P^{-1/2} + n_Q^{-1/2} & \text{for parametric }P(1|x) 
% \end{cases}  \]
% \end{enumerate}


% \paragraph{Concentration of (III)}
% Note that  \[ \begin{aligned}
% & \Bigg\|\widehat \bE_Q \bigg[\left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \Big\{\widehat \logit_P(x) -  \logit_P(x)  \Big\} \ddot \ell   \Big(  \tilde a(x), y  \Big)\bigg]\Bigg\|_2\\
% & \quad\le \widehat  \bE_Q \Bigg[\underbrace{\bigg\|\left(\begin{array}{c}
%      1 \\ x
% \end{array}\right)\bigg\|_2}_{\text{bounded }x} \Big|\widehat \logit_P(x) -  \logit_P(x)  \Big| \underbrace{\ddot \ell   \Big(  \tilde a(x), y  \Big)}_{\text{bounded curvature}}\Bigg] \\
% & \quad\le \widehat  \bE_Q \bigg[ \Big|\widehat \logit_P(x) -  \logit_P(x)  \Big| \bigg]\\
% & \quad\le \widehat  \bE_Q \bigg[ \Big|\widehat \logit_P(x) -  \logit_P(x)  \Big|, x \in [P_X] \bigg]\\
% & \quad \le  t \phi(n_P) 
% \end{aligned} \]  with probability $\ge 1-e^{-t^2}.$

% \paragraph{Concentration of (II)}
% For any $a\in \reals^{d+1}$ and $\|a\|_2 = 1$
% \[
% \begin{aligned}
% & a^T\widehat \bE_Q \bigg[ \underbrace{\left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \dot \ell \Big(  \logit_P(x) +  w^T x +  b, y  \Big)}_{u(x)}\bigg]\\
% & = a^T\widehat \bE_Q \bigg[ \left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \dot \ell \Big(  \logit_P(x) +  w^T x +  b, y  \Big)\bigg]\\
% & \qquad- a^T\underbrace{\bE_Q \bigg[ \left(\begin{array}{c}
%      1 \\ x
% \end{array}\right) \dot \ell \Big(  \logit_P(x) +  w^T x +  b, y  \Big)\bigg]}_{=0}\\
% & \le Ct n_Q^{-\frac12}
% \end{aligned}
% \]
% with probability $\ge 1-e^{-t^2}.$
% From the above inequality  \[ \Pr_{Q\text{-data}} \bigg( a^T\widehat \bE_Q\Big( u(x) - \bE_Q u(x)\Big) > t \bigg) \le \exp\big(-cn_Qt^2\big) \]
% Let  $\cN \subset \cS^{d}$  be the minimal set such that $\frac12\text{-net}(\cN) \supseteq \cS^{d}.$ Then 



\paragraph{Controlling (III):}  
\[
\begin{aligned}
& \Bigg|\widehat \bE_Q \bigg[ \nabla_{b}\nabla_w \ell \Big(  w_*^Tx,\tilde b(x)\Big) \big(\hat \eta_P(x) - \eta_P^*(x)\big)  \bigg]\Bigg| \\
& \le \widehat \bE_Q \bigg[ \nabla_{b}\nabla_w \ell \Big(  w_*^Tx,\tilde b(x)\Big) \Big|\hat \eta_P(x) - \eta_P^*(x)\Big| \bigg]\\
& \le \widehat \bE_Q \bigg[ \exp\Big(|w_*^Tx|\Big) \Big|\hat \eta_P(x) - \eta_P^*(x)\Big| \bigg]\\
& \le \widehat \bE_Q \bigg[ \exp\Big(D\|w_*\|_2\Big) \Big|\hat \eta_P(x) - \eta_P^*(x)\Big| \bigg]\\
& \le c_3t  n_P^{-\frac\beta{2\beta + d}} \exp\Big(D\|w_*\|_2\Big)
\end{aligned}
\] with probability $\ge 1 - e^{-t^2}.$

\paragraph{Controlling (I):}
Since \[ \bE_Q \Bigg[ \nabla_w \ell \Big(  w_*^Tx, \eta_P^*(x)\Big)  \Bigg] = 0, \] we have $\text{I} \le c_1t n_Q^{-1/2}$ with probability $\ge 1 - e^{-t^2}.$

\paragraph{Controlling (II):}

\[
\begin{aligned}
& \Bigg\| \widehat \bE_Q \bigg[ \nabla^2_w \ell \Big(  \tilde a(x), \eta_P^*(x)\Big)  \bigg] \big(\hat w - w\big)\Bigg\|_2 \\
& \ge\Bigg\| \bE_Q \bigg[ \nabla^2_w \ell \Big(  \tilde a(x), \eta_P^*(x)\Big)  \bigg] \big(\hat w - w\big)\Bigg\|_2 - c_2 t n_Q^{-\frac 12}\\
& =  \Bigg\|\bE_Q \bigg[ \nabla^2_w \ell \Big(  w_*^T x, \eta_P^*(x)\Big)  \bigg] \big(\hat w - w\big)\Bigg\|_2 -\Bigg\| \bE_Q \bigg[ \nabla^2_w \ell \Big(  \tilde a(x), \eta_P^*(x)\Big)  \bigg] \big(\hat w - w\big)\\
& \quad- \bE_Q \bigg[ \nabla^2_w \ell \Big(  w_*^T x, \eta_P^*(x)\Big)  \bigg] \big(\hat w - w\big)\Bigg\|_2 - c_2 t n_Q^{-\frac 12}\\
& \ge   \delta  \|\hat w - w\|_2 - c_4 D^3 \|\hat w - w\|_2^2 - c_2   t n_Q^{-\frac 12}
\end{aligned}
\] with probability $\ge 1 - e^{-t^2}.$

Hence with probability $\ge 1 - 3e^{-t^2}$ we have 
\[ 
\begin{aligned}
& \delta  \|\hat w - w\|_2 - c_4 D^3 \|\hat w - w\|_2^2 \le c_p' t n_Q^{-\frac 12} + c_n' t  n_P^{-\frac\beta{2\beta + d}}\\
\text{or,}\quad & \|\hat w - w\|_2 \le c_p t n_Q^{-\frac 12} + c_n t  n_P^{-\frac\beta{2\beta + d}}.
\end{aligned}\]

\input{lb}


\input{parametric}





\section{Upper Bound and classifier}

Look at the literature of partially linear regression model. 

\textbf{Idea}: Estimate the non-linear part of $\operatorname{logit}\text{-}\eta_Q(x)$ from combined data. This will hopefully give a correct estimate of the non-linear part. The linear part will be re-estimated anyway. 


\textbf{Q:} Does it work? (1) Does it make sense model-wise? (2) Check simulation. 


\subsection{Classification}


\paragraph{Estimation of logit:} (1) Get estimators $\tlogit(P)$ and $\tlogit(Q)$ from $P$ and $Q$ data; (2) Combine the logits to get the overall logit: \[ \tlogit = \rho \tlogit(P) + (1-\rho) \tlogit(Q).  \] 

\textbf{Q:} What does it estimate? Convergence of $\tlogit$?

(1) $\tlogit$ estimates $\logit = \rho\logit(P) + (1-\rho) \logit(Q). $
\paragraph{Linear model with interactions:} Here the logit is modeled linearly with non-linear interactions of covariates, \eg,\ $\logit(x_1, x_2) = \beta_0 + \beta_1 x_1 + \beta_2 x_2 + \beta_{1,1} x_1^2 + \beta_{1,2} x_1x_2.$ Hence the estimation of logits is equivalent to the estimations of the coefficient vectors. Under such parametric setup the choice of $\rho = \frac{n_P}{n_P + n_Q}$ and for such a choice \[ \tlogit =  \logit + (n_P + n_Q)^{-1/2} z  \] for some sub-Gaussain random variable $z$.


\paragraph{Non-parametric model:} Here we use the kernel to estimate the conditional probabilities $P(1|x)$ and $Q(1|x).$ To study the convergence property of $\tlogit$ we look at the following expansion 
\[
\begin{aligned}
\tlogit(x) & = \rho \log \Bigg(\frac 1 {n_P}\sum_{i = 1}^{n_P} y_i^{(P)} \frac1{h_P^d} K\Big(\frac{x - x_i^{(P)}}{h_P}\Big) \Bigg) - \rho \log \Bigg(\frac 1 {n_P}\sum_{i = 1}^{n_P} \big(1-y_i^{(P)}\big) \frac1{h_P^d} K\Big(\frac{x - x_i^{(P)}}{h_P}\Big) \Bigg)\\
& \quad + (1-\rho) \log \Bigg(\frac 1 {n_Q}\sum_{i = 1}^{n_Q} y_i^{(Q)} \frac1{h_Q^d} K\Big(\frac{x - x_i^{(Q)}}{h_Q}\Big) \Bigg)\\
& \quad - (1-\rho) \log \Bigg(\frac 1 {n_Q}\sum_{i = 1}^{n_Q} \big(1-y_i^{(Q)}\big) \frac1{h_Q^d} K\Big(\frac{x - x_i^{(Q)}}{h_Q}\Big) \Bigg)
\end{aligned}
\] 
Let's study the first term only. The Other three will follow similarly. Define \[ u_i = y_i^{(P)} \frac1{h_P^d} K\Big(\frac{x - x_i^{(P)}}{h_P}\Big). \] 
Note that \[\bbE[u_i] = \frac{1}{h_P^d}\int \eta_P(y) K\Big(\frac{x-y}{h}\Big) p_X(y) dy.  \]

From the literature of non-parametric functional estimation, setting $h_P = n_P^{-1/(2\beta + d)}$ we have
\[  \frac{1}{n_P}\sum_{i=1}^{n_P} u_i = \eta_P (x) + n_P^{-\frac{\beta}{2\beta + d}} z \] Use Taylor expansion we get \[ \tlogit =  \logit  + \left(\rho^2 n_P^{-\frac{2\beta}{2\beta + d}} + (1-\rho)^2 n_Q^{-\frac{2\beta}{2\beta + d}} \right) z.\]

\paragraph{Estimation of the linear shift}
Let us assume we know $\logit (x).$ Then the $Q$-population optimization problem is 
\[ 
\begin{aligned}
\hat \gamma & = \argmin\  \bbE_Q\left[ - y \big(\logit(x)+\gamma ^\top x\big) + \log \Big( 1+ \exp\big(\logit(x) + \gamma^\top x  \big)\Big) \right]\\
& = \argmin\  \bbE_{Q_X}\left[ - \eta_Q(x) \big(\logit(x)+\gamma ^\top x\big) + \log \Big( 1+ \exp\big(\logit(x) + \gamma^\top x  \big)\Big) \right]
\end{aligned}
 \]
 Noting that the expression under $\bbE_{P_X}$ is a cross-entropy term between  $\eta_Q(x)$ and $\expit\big(\logit(x) + \gamma^\top x\big)$, and $\logit(\eta_Q(x)) = \logit(x) + \rho w^\top x$ we conclude \[ \eta_Q(x) = \expit \big( \logit(x) + \gamma^\top x \big) \]
 
 
 
 \begin{lemma}[\cite{audibert2007fast}, Theorem 3.2]
 Let $\{(x_i, y_i)\}_{i=1}^n \in [0,1]^d \times \{0, 1\}$ are iid samples from $P \in \cP$. Then for $h = n^{-1/(2\beta + d)}$ and any $\delta>0$ we have \[
 \sup_{P\in \cP} \bbP\Big(\big|\hat \eta(x) - \eta(x)\big| > \delta \Big) \le C_1 \exp \Big(- C_2 n^{2\beta/(2\beta+d)}\delta^2\Big)
 \] for almost all $x$ w.r.t $P_X.$ 
 
 \end{lemma}
 
 Using the above lemma, for any $P\in \cP$ the random variables  $z_P = n_P^{\beta/(2\beta+d)}(\hat \eta_P(x) - \eta_P(x))$ and $z_Q = n_Q^{\beta/(2\beta+d)}(\hat \eta_Q(x) - \eta_Q(x))$ are independent sub-Gaussian. 
 
 Let us define 
 \begin{equation}
     \tilde \eta(x) = \expit \Big( \rho \logit \{\tilde \eta_P(x)\} + (1-\rho) \logit\{ \tilde \eta_Q(x)\} \Big)
     \label{eq:combined-reg-fn}
 \end{equation} and 
  \begin{equation}
      \eta(x) = \expit \Big( \rho \logit \{ \eta_P(x)\} + (1-\rho) \logit \{\eta_Q(x)\} \Big)
 \end{equation}
 
 Also define $a_P = n_P^{-\beta/(2\beta+d)}$ and $a_Q = n_Q^{-\beta/(2\beta+d)}.$ Since, $z_P$ and $z_Q$ are sub-Gaussian, there exists $c_1, c_2>0$ such that \[ 
 \bbP(|z_P| > t) \vee \bbP(|z_Q|>t) \le c_1 \exp \big(-c_2t^2\big)
 \] Hence, with probability $\ge 1 - 2 c_1 \exp \big(-c_2t^2\big)$ we have \[
 |z_P| \vee |z_Q| \le t.
 \]
 
 
 From \eqref{eq:combined-reg-fn} we have 
 \[ 
 \begin{aligned}
  \frac{\tilde \eta(x)}{1 - \tilde \eta(x)}&  = \left( \frac{\tilde \eta_P(x)}{ 1- \tilde \eta_P(x)} \right)^\rho \left( \frac{\tilde \eta_Q(x)}{ 1- \tilde \eta_Q(x)} \right)^{1-\rho}\\
  & = \left( \frac{ \eta_P(x) + a_P z_P}{ 1-  \eta_P(x) - a_P z_P} \right)^\rho \left( \frac{ \eta_Q(x) + a_Qz_Q}{ 1-  \eta_Q(x) - a_Qz_Q} \right)^{1-\rho}\\
  & \le \left( \frac{ \eta_P(x) + a_P (z_P)_+}{ 1-  \eta_P(x) - a_P (z_P)_+} \right)^\rho \left( \frac{ \eta_Q(x) + a_Q(z_Q)_+}{ 1-  \eta_Q(x) - a_Q(z_Q)_+} \right)^{1-\rho}
 \end{aligned}
 \]
 
 \begin{lemma}
 Let $0<\rho<1.$ Then the following inequality holds. 
\[
     \begin{aligned}
      (1+x)^\rho &  \le 1+\rho x ~~~\text{for any } x\ge 0,\\
      (1 - x)^\rho & \ge 1 - \rho x ~~~ \text{for any } 0 \le x \le 1.
     \end{aligned}
\]
 
 \end{lemma}

==> glm.tex <==

\section{Possible extensions}


\label{sec:extensions}
In this sections we present several avenues for related extensions on the linearly shifted posterior drift model.   A detailed exploration of these directions are not in the scope of this paper, but we present a short descriptions for each of these directions.  

\subsection{General regression setup}

In this section we present the posterior drift model and related studies for a generalized linear model (GLM). For a GLM let $\gamma$ bet the link function and $\mu_P(x)$ and $\mu_Q(x)$ are the conditional mean of $y$ given $x$ for distributions $P$ and $Q$ respectively, \ie, 
\[
\bbE_{\bbP} [y|x] = \mu_P(x), \quad \bbE_{\bbQ} [y|x] = \mu_Q(x).
\] We model the posterior drift  between $P$ and $Q$ as a linear transformation in a  lower dimensional feature space. For a $d_T$ dimensional  transformation $T(x)$ of the feature we define the posterior drift as
\begin{equation}
    \gamma(\mu_Q(x)) = \gamma(\mu_P(x)) + \beta^\top T(x).
    \label{eq:posterior-drift-glm}
\end{equation}

We describe the estimation procedure of the transfer parameter $\beta.$
As before we use an estimate of the source conditional mean $\mu_P(x)$ denoted as $\hat \mu_P(x).$ Let $\ell(y, a)$ be the negative log-likelihood for the particular GLM with response $y$ and conditional mean $a$. Given an estimate $\hat \mu_P(x)$ we  the transfer parameter $\beta$ is estimated  from the following optimization. 
\begin{equation}
\label{eq:optimization-transfer-glm}
    \hat \beta \in \argmin_{\beta} \frac1{n} \sum_{i=1}^n \ell\Big(y_{i}^{(Q)}, \gamma\big(\widehat\mu_P(x_i^{(Q)})\big) +  \beta^\top T\big(x^{(Q)}_{i}\big) \Big)\,.
\end{equation}

Using  $\hat \mu_P(x)$ and $\hat \beta$ one can estimate $\mu_Q(x)$ in the following way: $\hat \mu_Q (x) = \gamma^{-1} \big( \gamma(\hat \mu_P(x)) + \hat \beta^\top T(x) \big)$. Finally, using $\hat \eta_Q(x)$ one can make a prediction on the target response. 

Probably the simplest example is the linear link which corresponds to the normal distribution.  The negative log-likelihood for this example is $\ell(y, a, \tau) = \frac 12 \log(2\pi \tau^2) + \frac 1{2\tau^2} (y-a)^2. $ In such case one doesn't require to estimate the dispersion parameter (variance of normal distribution) for prediction. If estimation of $\tau$ is not required  the only relevant part of $\ell(y, a, \tau)$ is $\ell(y, a) \triangleq(y-a)^2$ and  the optimization problem \eqref{eq:optimization-transfer-glm} reduces to the least square regression problem
\[
\argmin_{\beta} \frac1{n} \sum_{i=1}^n \Big(y_{i}^{(Q)}-  \widehat\mu_P(x_i^{(Q)}) -  \beta^\top T\big(x^{(Q)}_{i}\big) \Big)^2\,. 
\] Finally,  the prediction rule is simply $\widehat\mu_P(x_i^{(Q)}) +  \hat \beta^\top T\big(x^{(Q)}_{i}\big).$

\subsection{High dimensional linear shift}

If $T(x)$ falls under the regime of high dimensional data the linearly shifted posterior drift model can easily accommodate  numerous techniques from the vast literature on high dimensional data. For example, one can estimate the coefficient for high dimensional linear shift by adding a regularization term $\cR(\beta)$ in the optimization \eqref{eq:optimization-transfer-glm}. 
\[
\hat \beta \in \argmin_{\beta} \frac1{n} \sum_{i=1}^n \ell\Big(y_{i}^{(Q)}, \gamma\big(\widehat\mu_P(x_i^{(Q)})\big) +  \beta^\top T\big(x^{(Q)}_{i}\big) \Big) + \cR(\beta)\,. 
\] An $\ell_1$-penalization (\cite{tibshirani1996regression}) on the above optimization can provide a model selection on the linear shift. Furthermore, under the sparsity assumption on the true value of $\beta$ one can establish model selection consistency (a similar result to lasso consistency \cite[Chapter 6]{buhlmann2011statistics}) on $\hat \beta$. 

\subsection{Non-parametric estimation of the link function}

In this paper we mainly concern ourselves with prediction on the target data which is known to be robust mis-specification on the link function. In fact, in our simulation we validate this fact: we show that if the data generative link differs from the link considered in model fitting process the behavior of prediction is not that different from the case of  well-specified link. But for a mis-specified link the optimizations \eqref{eq:offset-estimate} and \eqref{eq:optimization-transfer-glm} often produce a biased estimate on the linear shift coefficient $\beta$. This could be problematic if one is interested to characterize the difference between source and target populations and draw inference on $\beta$. In such case one may require to consider the non-parametric estimation of the link function. [SM: Mouli da please write this; about single index type model]. 


==> lb.tex <==
\section{Lower bound}

Main assumptions: \begin{enumerate}
    \item $\beta$ H\"older smoothness for $\eta_Q$:
    \[ \Big|\eta_Q(x) - \lfloor \beta \rfloor \text{-order Taylor expansion of }\eta_{Q}(x)\text{ at }y\Big| \le C_\beta \|x- y\|_2^\beta \]
    \item $\alpha$ margin condition for $\eta_Q(x)$:
    \[ P_X\Big(\big| \eta_Q(x) - 1/2  \big|\le t\Big) \le C_\alpha t^\alpha \]
\end{enumerate}
\begin{theorem}[Informal]
\[\inf_{\hat f} \sup_{(P, Q) \in \Pi} \ge c \left( (n_P + n_Q)^{-\frac\beta{2\beta + d}} +  n_Q^{-1/2} \right)^{{1+\alpha}} \]
\end{theorem}



\subsection{Proof of Lower bound (non-parametric model)}
\paragraph{Non-parametric part}
Set the shift $w = 0$, which leads to $\eta_P  = \eta_Q$ with combined sample size $n_P + n_Q.$ Then apply standard technique to get \[\inf_{\hat f} \sup_{(P, Q) \in \Pi} \ge c  (n_P + n_Q)^{-\frac{\beta(1+\alpha)}{2\beta + d}}. \]



 Let $r = c_r (n_P+n_Q)^{-1/(2\beta + d)}, m = \lfloor c_m r ^{\alpha\beta - d}\rfloor,$ where $\alpha\ge 0 $ is the noise condition exponent and $\beta>0 $ is the H\"older smoothness exponent. Also, define $w = c_w r^d$ where $c_r = (1/17) \wedge (1/6 (3C_\beta/2)^{-1/\beta} ), c_m = 8 \times 17^{\alpha\beta - d}$ and $c_w \in (0, 1]$ is a constant to be picked later. The preceding constants satisfy \[ 8 \le m <\frac12 \left\lfloor \frac 1r \right\rfloor^d. \]  To see the first inequality, we observe that $r \le 1/17$ and recall $\alpha\beta \le d.$ Thus \[ m = 8 \times (17r)^{\alpha\beta - d} \ge 8. \] To see the second inequality, we observe that $r^{-1} \ge 16,$ which implies $r^{-1}\le 17\lfloor r^{-1}\rfloor/16.$ Thus \[ m = 8 (17r)^{\alpha\beta} \left(\frac 1{17r}\right)^d \le 8\cdot  16^{-d} \lfloor r^{-1} \rfloor ^d \le\frac1 2 \lfloor r^{-1} \rfloor ^d. \] We also have $2mw = 2mc_w r^d<1. $
    
    \textit{Construction of $\{\Pi_i\}_{i=1}^M$.}
    Let $r_1 = 1/\lfloor 1/r\rfloor.$ Let us consider the grid of points \begin{equation}
        \cZ = \{ (1/2+i)r_1 : i = 0, 1, \dots , \lfloor 1/r\rfloor -1 \}^d.
    \end{equation} 
    We see that $\cZ$ is a grid of equally spaced points of size $\lfloor 1/r \rfloor^d.$ For a $z \in \cZ$ we consider the hyper-cube \[ C(z) = \{x \in [0,1]^d: \|x-z\|_\infty\le r_1/2 \}. \] Note that, volume of each of these hyper-cubes is $r_1^d.$ Let $\cZ_1, \cZ_2 \subset \cZ $ be subsets of size $m$. Moreover, we let $\cZ_1 $ and $\cZ_2$ are disjoint. We define a bijection $u : \cZ_1 \to \cZ_2 $ which shall be used to construct the conditional densities. We define $\cZ_0 = \cZ \backslash (\cZ_1 \cup \cZ_2).$ On this grid, we define a set of distributions parametrized by $\sigma\in \{ -1, 1 \}^{\cZ_1}.$
    
     \noindent\textit{Conditional densities.} Let $k\in (0, 1/2)$ be a number which will be decided later. Let $R_+ = [0, \infty)$ and $u_\beta : \reals_+ \to \reals$ such that: 
    If $\beta <1,$ we define
    \[ u_\beta(x) = \begin{cases} 
    \big( 1-x \big)^{\beta} & \text{if}\  x \le 1\\
    0 & \text{otherwise,}
    \end{cases} \] 
    
    If $\beta \ge 1,$ we define
    \[ u_\beta(x) = \begin{cases} 
    \big( 2^{1-\beta}-x^\beta \big) & \text{if}\  x \le 1/2\\
    \big( 1 -x \big)^\beta & \text{if}\  1/2 < x \le 1\\
    0 & \text{otherwise,}
    \end{cases} \] 
    
    
 
    
    and \[ v(x) = \begin{cases} 
     \mu'( 1-2x )^{\beta} & \text{if}\  x \le 1/2\\
     0 & \text{otherwise.}
     \end{cases} \]
    
   
    
    It can be shown that $u$ is $\beta$-smooth with constant $L.$   Recall $C_\beta' = (C_\beta L^{-1})\wedge (1/3).$ Therefore, the following functions are $(C_\beta, \beta)$-H\"older: 
    \[ z \in \cZ_1, \hspace{0.3cm} \eta_z(x) = C_\beta' r_1^\beta u_\beta \left(\frac{2\|x-z\|_2 }{c_wr_1}\right). \]
    
    For a parameter $\sigma$ the  construction of  conditional probabilities and marginal density of $X$ given below. 
    
    
   
    
    
    \begin{equation}
    \label{eq:conditional-prob}
    \eta_P^{\sigma}(x) = \eta_Q^{\sigma}(x) =    \begin{cases}
   \frac12 \Big( 1+  \sigma(z) \eta_z(x)\Big) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
   \frac12 \Big( 1-  \sigma(z)  \eta_{f(z)}(x)\Big) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    \frac12  & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0,
    \end{cases} 
    \end{equation} and 
    \begin{equation}
        p_X  = q_X \equiv 1
    \end{equation}
  
    
    
   
    \begin{equation}
    \begin{aligned}
    P^{\sigma}( X \in A, Y = y) &  =   Q^{\sigma}( X \in A, Y = y)\\ &  = \int_A [\eta_P^\sigma(x)\indicator(y = 1) + (1-\eta_P^\sigma(x))  \indicator (y = 0) ] p_X(x) dx.
    \end{aligned}
        \label{eq:dist-Q}
    \end{equation}
    Given the source and target distributions we define the joint distribution as \begin{equation}
        \label{eq:dist-joint}
        \Pi_\sigma = P_\sigma^{\otimes n_P} \otimes Q_\sigma ^{\otimes n_Q}
    \end{equation}
    
    Here,  $\Omega = [0,1]^d$ is a regular set and $q^\sigma _X = p_X \equiv 1$, which satisfies strong density assumption. We refer to lemma \ref{lemma:margin-bound}, where it is shown $Q_\sigma$ satisfies $\alpha$-margin condition with constant $C_\alpha.$
   

        
 
        
        For such a construction we notice that \begin{align*}
            \cE_{Q^\sigma}(h) & = 2\Ex _{Q_X} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( h(X) \neq h^*_\sigma(X)  \right)\right]\\
	& \ge c' r^\beta Q_X\left( \{h(X) \ne h_\sigma^*(X)  \}  \right)
        \end{align*}
        
        
    Let $ \cF $ be the set of all classifier relevant to this classification problem. For $\sigma \in \{-1, 1\}^{\cZ_1}$ let  $h_\sigma$ be the Bayes classifier corresponding to the probability distribution $Q_\sigma$ defined as $ h_\sigma (x) = \indicator\{\eta_{ Q_\sigma }(x) \ge 1/2\}.$  For $ \sigma,\sigma'\in\{-1, 1\}^{\cZ_1} $ define $ \bar\rho (\sigma,\sigma') = \cE_{\sigma} (h_{\sigma'})   $ and  $\rho(\sigma,\sigma') = \text{card} \{z\in\cZ_1 :\sigma(z) \neq \sigma'(z) \} $ as the Hamming distance. Then \begin{align*}
        \bar\rho (\sigma,\sigma') & = 2\Ex _{Q_{\sigma, X}} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( h_\sigma(X) \neq h_{\sigma'}(X)  \right)\right]\\
        & \ge c' r_1^\beta Q_{\sigma, X }\left( \{h_\sigma(X) \ne h_{\sigma'}(X)  \}  \right)\\
         & \ge c'c_w r_1^\beta \left( \frac {r_1}2 \right)^d \rho(\sigma, \sigma').
    \end{align*}
	
	
	
	Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m  $ be the choice obtained from the  lemma 6.2 in main paper. For each $ i \in \{0,\ldots,M\} $ let us set the joint distribution of  $ (\bX,\bY) $ as $ \Pi_i = {P_{\sigma_i}}^{\otimes n_p} \otimes {Q_{\sigma_i}}^{\otimes n_Q} .$ Note that for such a choice $\rho(\sigma_i, \sigma_j) \ge m/8$ whenever $i\neq j.$
	
	Then  \begin{align*}
	\bar\rho (\sigma_i, \sigma_j) &\ge c'c_w r_1^\beta \left( \frac {r_1}2 \right)^d \frac m8\\ 
	&\ge \frac{c'c_wc_m}{2^{d}}  r_1^\beta r_1^d    r_1^{\alpha\beta -d}  \\
	& \ge C' r_1^{\beta (1+\alpha)}\\
	& = C ( n_P+n_Q)^{-\frac{\beta(1+\alpha)}{2\alpha + d}}\\
	& \triangleq 2s
	\end{align*}
	for some $C>0.$
	
	
	
	Now we bound the Kulback-Leibler divergence between the joint distributions $\Pi_{\sigma_i}.$ Using lemma \ref{lemma:kl-distance-joint} we get 
	\begin{align*}
	KL(\Pi_{\sigma_i}|| \Pi_{\sigma_j}) & \le 2c_w^dK(d, \alpha, \beta)c_r^{2\beta + d}\rho(\sigma_i, \sigma_j) \\
	& \le  2c_w^dK(d, \alpha, \beta)c_r^{2\beta + d}m \\
	& \le \frac 19 \log_2(M) \\
	\end{align*}
	for suitable $c_w < 1.$
	

	
	
	
	Finally we appeal to proposition 6.1 in main paper (and Markov's inequality) to obtain the minimax rate \begin{align*}
\sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
& \ge s \sup_{\sigma\in \{-1,1\}^{\cZ_1}} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
& \ge s \frac {3-2\sqrt{2}}{8}\\
& \ge C(n_P + n_Q)^{-\frac{\beta(1+\alpha)}{2\beta + d}}.
\end{align*}


    


\paragraph{Parametric part} Setting $\logit(\eta_P(x)) = 0$ and $w_\sigma = \frac\sigma {\sqrt{n_Q}}$ where $\sigma \in \{-1, 1\}^{\otimes d}$ 
 we get $\logit(\eta_Q^\sigma(x)) = \frac{\sigma^\top x} {\sqrt{n_Q}}$
Then we should get 
\[\inf_{\hat f} \sup_{(P, Q) \in \Pi} \ge c  \left(\frac d {n_Q}\right)^{-\frac{1+\alpha}{2}}. \]





\section{Upper Bound and classifier}

Look at the literature of partially linear regression model. 

\textbf{Idea}: Estimate the non-linear part of $\operatorname{logit}\text{-}\eta_Q(x)$ from combined data. This will hopefully give a correct estimate of the non-linear part. The linear part will be re-estimated anyway. 


\textbf{Q:} Does it work? (1) Does it make sense model-wise? (2) Check simulation. 


\subsection{Classification}


\paragraph{Estimation of logit:} (1) Get estimators $\tlogit(P)$ and $\tlogit(Q)$ from $P$ and $Q$ data; (2) Combine the logits to get the overall logit: \[ \tlogit = \rho \tlogit(P) + (1-\rho) \tlogit(Q).  \] 

\textbf{Q:} What does it estimate? Convergence of $\tlogit$?

(1) $\tlogit$ estimates $\logit = \rho\logit(P) + (1-\rho) \logit(Q). $
\paragraph{Linear model with interactions:} Here the logit is modeled linearly with non-linear interactions of covariates, \eg,\ $\logit(x_1, x_2) = \beta_0 + \beta_1 x_1 + \beta_2 x_2 + \beta_{1,1} x_1^2 + \beta_{1,2} x_1x_2.$ Hence the estimation of logits is equivalent to the estimations of the coefficient vectors. Under such parametric setup the choice of $\rho = \frac{n_P}{n_P + n_Q}$ and for such a choice \[ \tlogit =  \logit + (n_P + n_Q)^{-1/2} z  \] for some sub-Gaussain random variable $z$.


\paragraph{Non-parametric model:} Here we use the kernel to estimate the conditional probabilities $P(1|x)$ and $Q(1|x).$ To study the convergence property of $\tlogit$ we look at the following expansion 
\[
\begin{aligned}
\tlogit(x) & = \rho \log \Bigg(\frac 1 {n_P}\sum_{i = 1}^{n_P} y_i^{(P)} \frac1{h_P^d} K\Big(\frac{x - x_i^{(P)}}{h_P}\Big) \Bigg) - \rho \log \Bigg(\frac 1 {n_P}\sum_{i = 1}^{n_P} \big(1-y_i^{(P)}\big) \frac1{h_P^d} K\Big(\frac{x - x_i^{(P)}}{h_P}\Big) \Bigg)\\
& \quad + (1-\rho) \log \Bigg(\frac 1 {n_Q}\sum_{i = 1}^{n_Q} y_i^{(Q)} \frac1{h_Q^d} K\Big(\frac{x - x_i^{(Q)}}{h_Q}\Big) \Bigg)\\
& \quad - (1-\rho) \log \Bigg(\frac 1 {n_Q}\sum_{i = 1}^{n_Q} \big(1-y_i^{(Q)}\big) \frac1{h_Q^d} K\Big(\frac{x - x_i^{(Q)}}{h_Q}\Big) \Bigg)
\end{aligned}
\] 
Let's study the first term only. The Other three will follow similarly. Define \[ u_i = y_i^{(P)} \frac1{h_P^d} K\Big(\frac{x - x_i^{(P)}}{h_P}\Big). \] 
Note that \[\bbE[u_i] = \frac{1}{h_P^d}\int \eta_P(y) K\Big(\frac{x-y}{h}\Big) p_X(y) dy.  \]

From the literature of non-parametric functional estimation, setting $h_P = n_P^{-1/(2\beta + d)}$ we have
\[  \frac{1}{n_P}\sum_{i=1}^{n_P} u_i = \eta_P (x) + n_P^{-\frac{\beta}{2\beta + d}} z \] Use Taylor expansion we get \[ \tlogit =  \logit  + \left(\rho^2 n_P^{-\frac{2\beta}{2\beta + d}} + (1-\rho)^2 n_Q^{-\frac{2\beta}{2\beta + d}} \right) z.\]

\paragraph{Estimation of the linear shift}
Let us assume we know $\logit (x).$ Then the $Q$-population optimization problem is 
\[ 
\begin{aligned}
\hat \gamma & = \argmin\  \bbE_Q\left[ - y \big(\logit(x)+\gamma ^\top x\big) + \log \Big( 1+ \exp\big(\logit(x) + \gamma^\top x  \big)\Big) \right]\\
& = \argmin\  \bbE_{Q_X}\left[ - \eta_Q(x) \big(\logit(x)+\gamma ^\top x\big) + \log \Big( 1+ \exp\big(\logit(x) + \gamma^\top x  \big)\Big) \right]
\end{aligned}
 \]
 Noting that the expression under $\bbE_{P_X}$ is a cross-entropy term between  $\eta_Q(x)$ and $\expit\big(\logit(x) + \gamma^\top x\big)$, and $\logit(\eta_Q(x)) = \logit(x) + \rho w^\top x$ we conclude \[ \eta_Q(x) = \expit \big( \logit(x) + \gamma^\top x \big) \]
 
 
 
 \begin{lemma}[\cite{audibert2007fast}, Theorem 3.2]
 Let $\{(x_i, y_i)\}_{i=1}^n \in [0,1]^d \times \{0, 1\}$ are iid samples from $P \in \cP$. Then for $h = n^{-1/(2\beta + d)}$ and any $\delta>0$ we have \[
 \sup_{P\in \cP} \bbP\Big(\big|\hat \eta(x) - \eta(x)\big| > \delta \Big) \le C_1 \exp \Big(- C_2 n^{2\beta/(2\beta+d)}\delta^2\Big)
 \] for almost all $x$ w.r.t $P_X.$ 
 
 \end{lemma}
 
 Using the above lemma, for any $P\in \cP$ the random variables  $z_P = n_P^{\beta/(2\beta+d)}(\hat \eta_P(x) - \eta_P(x))$ and $z_Q = n_Q^{\beta/(2\beta+d)}(\hat \eta_Q(x) - \eta_Q(x))$ are independent sub-Gaussian. 
 
 Let us define 
 \begin{equation}
     \tilde \eta(x) = \expit \Big( \rho \logit \{\tilde \eta_P(x)\} + (1-\rho) \logit\{ \tilde \eta_Q(x)\} \Big)
     \label{eq:combined-reg-fn}
 \end{equation} and 
  \begin{equation}
      \eta(x) = \expit \Big( \rho \logit \{ \eta_P(x)\} + (1-\rho) \logit \{\eta_Q(x)\} \Big)
 \end{equation}
 
 Also define $a_P = n_P^{-\beta/(2\beta+d)}$ and $a_Q = n_Q^{-\beta/(2\beta+d)}.$ Since, $z_P$ and $z_Q$ are sub-Gaussian, there exists $c_1, c_2>0$ such that \[ 
 \bbP(|z_P| > t) \vee \bbP(|z_Q|>t) \le c_1 \exp \big(-c_2t^2\big)
 \] Hence, with probability $\ge 1 - 2 c_1 \exp \big(-c_2t^2\big)$ we have \[
 |z_P| \vee |z_Q| \le t.
 \]
 
 
 From \eqref{eq:combined-reg-fn} we have 
 \[ 
 \begin{aligned}
  \frac{\tilde \eta(x)}{1 - \tilde \eta(x)}&  = \left( \frac{\tilde \eta_P(x)}{ 1- \tilde \eta_P(x)} \right)^\rho \left( \frac{\tilde \eta_Q(x)}{ 1- \tilde \eta_Q(x)} \right)^{1-\rho}\\
  & = \left( \frac{ \eta_P(x) + a_P z_P}{ 1-  \eta_P(x) - a_P z_P} \right)^\rho \left( \frac{ \eta_Q(x) + a_Qz_Q}{ 1-  \eta_Q(x) - a_Qz_Q} \right)^{1-\rho}\\
  & \le \left( \frac{ \eta_P(x) + a_P (z_P)_+}{ 1-  \eta_P(x) - a_P (z_P)_+} \right)^\rho \left( \frac{ \eta_Q(x) + a_Q(z_Q)_+}{ 1-  \eta_Q(x) - a_Q(z_Q)_+} \right)^{1-\rho}
 \end{aligned}
 \]
 
 \begin{lemma}
 Let $0<\rho<1.$ Then the following inequality holds. 
\[
     \begin{aligned}
      (1+x)^\rho &  \le 1+\rho x ~~~\text{for any } x\ge 0,\\
      (1 - x)^\rho & \ge 1 - \rho x ~~~ \text{for any } 0 \le x \le 1.
     \end{aligned}
\]
 
 \end{lemma}

==> parametric.tex <==
\section{Parametric setup}

In this section we consider the parametric evaluation of the posterior drift model rates. Let $\mu$ as a probability measure defined on the space $\reals^d \times \{0, 1\}$ (appropriate for classification data). For $\reals^d \times \{0, 1\} \ni  (x, y) \sim \mu $ we assume the marginal $\mu_x$ has Lebesgue density.  In the parametric setup our goal is to estimate the best approximation (projection in entropy loss divergence) of the logit function $\logit_{\mu}(x) \triangleq  \log \big(\mu(y = 1\mid x)/\mu(y = 0\mid x)\big)$ in a function subspace \[
V = \Bigg\{ \sum_{j = 1}^s a_j \psi_j: a_j \in \reals  \Bigg\}.
\] 
To be more specific we want to estimate the function \[
\bP_{V, \mu} \big( \logit_\mu\big) = {\beta^{(\mu)}_V}^\top  \psi_V
\] where $\psi_V = (\psi_1 , \dots , \psi_s)^\top$ and \[
\beta^{(\mu)}_V= \underset{\beta \in \reals^s}{\argmin} ~ \bbE_\mu \Big[\ell\big(\beta^\top \psi_V(x), y\big)\Big]
\] for the entropy-loss $\ell(a, y) = -ya + \log(1 + e^a).$ We let $\cP$ as the collection of such probability distributions $\mu$, with some more restrictions (to be defined later). 

For some integer $0 < s_0 < s$ let $V_0 \triangleq \text{span}\big( \{ \psi_j\mid j = 1, \dots s_0 \} \big) \subseteq V$ be a function-subspace. We define the collection of posterior drifts (on $V_0$) as $\operatorname{PD}(V_0) \subseteq \cP ^2 $ such that for any $(P, Q) \in \operatorname{PD}(V_0)$ the following condition is satisfied.
\begin{equation}
    \label{eq:posterior-drift}
    \logit_P - \bP_{V_0, P} \big( \logit_P \big) = \logit_Q - \bP_{V_0, Q} \big( \logit_Q \big).
\end{equation}


Let $\{(x_i, y_i)\}_{i = 1}^{n_P} \sim_{\iid} P.$ Let \[
\widehat\beta^{(P)}_V= \underset{\beta \in \reals^s}{\argmin} ~ \bbE_{\bbP_n} \Big[\ell\big(\beta^\top \psi_V(x), y\big)\Big].
\] The optimality condition for the above minimization is:
\[
{\Big\{\nabla_{\beta} L_{\bbP_n}\big(\widehat\beta^{(P)}_V\big)\Big\}}^\top\big(\beta - \widehat\beta^{(P)}_V\big) \ge 0, ~~ \forall \beta.
\] 

We decompose the above optimality condition as 
\[
\begin{aligned}
0 \le &  {\Big\{\nabla_{\beta} L_{\bbP_n}\big(\widehat\beta^{(P)}_V\big)\Big\}}^\top\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)\\
= & {\Big\{\nabla_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\}}^\top\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big) - \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\widetilde\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)
\end{aligned}
\] or \[
\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\widetilde\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big) \le {\Big\{\nabla_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\}}^\top\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big).
\]
Here, 
\[
\begin{aligned}
& \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\widetilde\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big) \\
 = & \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)\\
 & + \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\widetilde\beta^{(P)}_V\big) - \nabla^2_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)\\
 & = (I) + (II)
\end{aligned}
\]

Now, \[
\begin{aligned}
|(II)| = &  \Bigg|\frac1 {n_P}\sum_{i = 1}^{n_P}  \Big[ \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \psi_V(x_i)\Big]^2 \Big[ \ddot \rho\big(\psi_V(x)^\top {\widetilde\beta^{(P)}_V} \big) - \ddot \rho\big(\psi_V(x)^\top {\beta^{(P)}_V} \big) \Big]\Bigg|\\
\le & \frac1 {n_P}\sum_{i = 1}^{n_P}  \Big| \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \psi_V(x_i)\Big|^3 \\
\le & \big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2^3\Bigg( \frac1 {n_P}\sum_{i = 1}^{n_P} \|\psi_V(x_i)\|_2^3 \Bigg)
\end{aligned}
\]

To get a lower bound on (I) we notice that 
\[
\begin{aligned}
a^\top \nabla^2_{\beta}\ddot \rho \big( \psi_V(x)^\top \beta^{(P)}_V\big) a = & \big(a^\top \psi_V(x) \big)^2 \frac{\exp\big( \psi_V(x)^\top \beta^{(P)}_V\big)}{\Big(1 + \exp\big( \psi_V(x)^\top \beta^{(P)}_V\big)\Big)^2}\\
= & \big(a^\top u  \big)^2 r^2 \frac{\exp\big( u^\top \beta^{(P)}_V r\big)}{\Big(1 + \exp\big( u^\top \beta^{(P)}_V r\big)\Big)^2}
\end{aligned}
\]
for $r = \|\psi_V(x)\|_2$ and $u = \psi_V(x)/r.$ Without loss of generality we assume $u^\top \beta^{(P)}_V\ge 0.$ Otherwise, replace $u^\top \beta^{(P)}_V$ with $-u^\top \beta^{(P)}_V$ (since $e^a/(1+e^a)^2 = e^{-a}/(1+e^{-1})^2$). 
We notice that $r^2 \exp\big( u^\top \beta^{(P)}_V r\big)/\Big(1 + \exp\big( u^\top \beta^{(P)}_V r\big)\Big)^2$ is bounded (by some $M>0$) with respected to $r.$ Hence, we conclude $a^\top \nabla^2_{\beta}\ddot \rho \big( \psi_V(x)^\top \beta^{(P)}_V\big) a \le M\|a\|_2^2. $ Finally from Bernstein inequality we conclude that 
\[
\begin{aligned}
(I) =&  \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big) \\
=&  \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big) - \nabla^2_{\beta} L_{\bbP}\big(\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)\\
& +  \big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)^\top \Big\{\nabla^2_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\}\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big)\\
& \ge \Big(\alpha - \frac{3Mt}{\sqrt{n_P}}\Big)\big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2^2
\end{aligned}
\] with probability $\ge 1 - \exp(-t^2)$

Hence, 
\[
\begin{aligned}
\Big(\alpha - \frac{3Mt}{\sqrt{n_P}}\Big) \big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2^2 - M_3 \big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2^3 \le \Big\|\nabla_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\|_2\big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2
\end{aligned}
\]
or \[ 
\Big(\alpha - \frac{3Mt}{\sqrt{n_P}}\Big) \big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2 - M_3 \big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2^2 \le \Big\|\nabla_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\|_2
\]

This implies either $\big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2 \le C \Big\|\nabla_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\|_2$ or $\big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2 \ge c$ for some $c, C>0.$ From the consistency of M-estimators we get the rate
\[
\big\|\big(\beta^{(P)}_V - \widehat\beta^{(P)}_V\big\|_2 \le C \Big\|\nabla_{\beta} L_{\bbP_n}\big(\beta^{(P)}_V\big)\Big\|_2 \le C't \sqrt{\frac s{n_P}}
\]
 with probability $\ge 1 - 2e^{-t^2}.$
